Scalable Neural Network Training over Distributed Graphs

Graph neural networks (GNNs) fuel diverse machine learning tasks involving graph-structured data, ranging from predicting protein structures to serving personalized recommendations. Real-world graph data must often be stored distributed across many machines not just because of capacity constraints, but because of compliance with data residency or privacy laws. In such setups, network communication is costly and becomes the main bottleneck to train GNNs. Optimizations for distributed GNN training have targeted data-level improvements so far -- via caching, network-aware partitioning, and sub-sampling -- that work for data center-like setups where graph data is accessible to a single entity and data transfer costs are ignored. We present RETEXO, the first framework which eliminates the severe communication bottleneck in distributed GNN training while respecting any given data partitioning configuration. The key is a new training procedure, lazy message passing, that reorders the sequence of training GNN elements. RETEXO achieves 1-2 orders of magnitude reduction in network data costs compared to standard GNN training, while retaining accuracy. RETEXO scales gracefully with increasing decentralization and decreasing bandwidth. It is the first framework that can be used to train GNNs at all network decentralization levels -- including centralized data-center networks, wide area networks, proximity networks, and edge networks.

==> algorithms/fl.tex <==
\begin{algorithm}[t]
% \SetAlgoLined
% \SetKwInOut{Input}{Input}
% \SetKwInOut{Output}{Output}
\caption{$\cf{FederatedLearning}$: Outline of the federated learning protocol to train an \mlp in \toolgnn}
\label{alg:fl}
\begin{algorithmic}[1]
\STATE {\bfseries Input:} Server, Clients, message-passing round number: $\hopiter$, \# training rounds: $R$

\textit{// initialize server and clients}
\STATE {Server:} \{$\set{V}$, $\set{V}^{tr}$, $\set{V}^{val}$, $\set{V}^{test}$, $\fc{f}_{\theta}$, $\num$, $\numrounds$\}
\STATE {Clients:} [\{$v$, $nei$:$\set{N}(v)$, $feat$:$\arr{F}[v]$, $label$:$\arr{L}[v]$, $Opt$\} $\forall v \in [|\set{V}|]$]
\item[]\item[]
\textit{//To train model number m} 
\STATE {\bfseries Server executes:}
    \STATE\hspace*{\myindent} $\text{\mlp}_m$ = $\fc{f}^{\hopiter-1}_{\theta}$
    \STATE\hspace*{\myindent} $\cf{initModel}(\text{\mlp}_m)$ \textit{// initialize the model}
    \item[]
    \begin{ALC@g}
        \FOR{$i=0$ to $i=R-1$}
            \STATE $\set{V}^{tr}_s, \set{V}^{val}_s=\cf{sampleNodes}(\set{V}^{tr}, \set{V}^{val})$ \textit{// sample sets of training and validation clients}
            \STATE $\cf{sendMessage}(\set{V}^{tr}_s, \text{\mlp}_m, \text{``train''})$
            \STATE $\cf{sendMessage}(\set{V}^{val}_s, \text{\mlp}_m, \text{``validation''})$
            \item[]
            \STATE $\text{\mlp}^j_m$, $client_j$ = $\cf{receiveMessage()}$ \textit{// wait for the replies from all clients}
            \item[]
            \STATE // On receiving all updated local models
            \STATE $\text{\mlp}^{agg}_m = \frac{\sum_{j=0}^{j=|\set{V}^{tr}_s|} \text{\mlp}^{j}_m}{|\set{V}^{tr}_s|}$
            \STATE$\text{\mlp}_m = \text{\mlp}^{agg}_m$
        \ENDFOR
    \end{ALC@g}
    \STATE\hspace*{\myindent} {\bfseries Output:}{Trained $\text{\mlp}_m$}
\item[]
\STATE {\bfseries Each client executes:}
    \STATE\hspace*{\myindent} $\text{\mlp}_m, task$ = $receiveMessage()$
    % \bindent
    \begin{ALC@g}
        \IF{$task$ is \text{``train''}}
            \STATE $\text{\mlp}^{tr}_m = \cf{trainModel}(\text{\mlp}_m, feat, label, Opt)$
            \STATE $\cf{sendMessage}(server, \text{\mlp}^{tr}_m)$
        \ENDIF
    \end{ALC@g}
    \STATE \hspace*{\myindent}\textit{// for validation compute accuracy and send it back}
\end{algorithmic}
\end{algorithm}

==> algorithms/messagep.tex <==
\begin{algorithm}[t]
\caption{$\cf{AsyncMessagePassing}$: Outline of message-passing round to train \toolgnn}
\label{alg:messagep}
\begin{algorithmic}[1]
\STATE {\bfseries Input:} Clients, $timeout$, message-passing round number: $\hopiter$
\STATE {Clients:} [\{$v$, $nei$:$\set{N}(v)$, $feat$:$\arr{F}[v]$, $label$:$\arr{L}[v]$, $Opt$\} $\forall v \in [|\set{V}|]$\}]

\item[]\item[]
\textit{// For message-passing round number m}
\STATE {\bfseries Each client ($v$) executes:}
    \STATE\hspace*{\myindent} $Q^m$ = $\cf{computeEmbedding(m)}$ \textit{// Computes $m^{th}$ embedding}
    \begin{ALC@g}
        \WHILE{not $timeout$}
            \STATE\textit{// scan for available client-to-client communication channels}
            \STATE $clients\_available$ = $\cf{scanForClients()}$ 
            \item[]
            \FOR{$u$ in $clients\_available$}
                \IF{$u \in \set{N}(v)$}
                    \STATE $conn$ = $\cf{initConnection(u)}$
                    \STATE \textit{// send and receive embeddings}
                    \STATE $conn.\cf{sendEmbedding}(Q^m)$
                    \STATE $Q_u^m$ = $conn.\cf{recvEmbedding()}$
                    \STATE $conn.close()$ \textit{// close connection}
                \ENDIF
            \ENDFOR
        \ENDWHILE
    \end{ALC@g}
%     \begin{ALC@g}
%         \FOR{$u$ in $\set{N}(v)$}
        
%         \ENDFOR
%     \end{ALC@g}
%     \ENDWHILE
% \FOR{$client$ in Clients}
%     \STATE \textit{// Computes $m^{th}$ embedding}
%     \STATE $client.Q^m$ = $\cf{client.computeEmb(m)}$
% \ENDFOR

% \WHILE{not $timeout$}
%     \FOR{$client$ in Clients}
%         \FOR{$client\_nei$ in $client.neighbors$}
%             \STATE \textit{// if $client$ \& $client\_nei$ are in proximity}
%             \IF{$\cf{Contact}(client, client\_nei)$}
%                 \STATE \textit{send and receive embeddings}
%                 \STATE $client.\cf{sendEmbedding}(client\_nei, client.Q^m)$
%             \ENDIF
%         \ENDFOR
%     \ENDFOR
% \ENDWHILE
\end{algorithmic}
\end{algorithm}

==> algorithms/outline.tex <==
\begin{algorithm}[t]
\scriptsize
\caption{Outline of training a \toolgnn}
\label{alg:outline}
\begin{algorithmic}[1]
\STATE {\bfseries Input:} $\set{V}$, Train-val-test nodes: $\set{V}^{tr}$-$\set{V}^{val}$-$\set{V}^{te}$, features: $\arr{F}$, labels: $\arr{L}$, model: $\fc{f}_\theta$, optimizer: $Opt$, max hops: $\num$, \# training rounds: $\numrounds$, message-passing timeout: $timeout$

\textit{// initialize server and clients}
\STATE \textbf{Server}: \{$\set{V}$, $\set{V}^{tr}$, $\set{V}^{val}$, $\set{V}^{test}$, $\fc{f}_{\theta}$, $\num$, $\numrounds$\}
\STATE {\bfseries Clients}: [\{$v$, $nei$:$\set{N}(v)$, $feat$:$\arr{F}[v]$, $label$:$\arr{L}[v]$, $Opt$\} $\forall v \in [|\set{V}|]$]

\FOR{$\hopiter=0$ {\bfseries to} $\hopiter=\num$}

    \IF{$\hopiter>0$}
    \STATE \textit{// server syncs previous trained model with all nodes and starts $\hopiter^{th}$ message-passing round}
    \STATE $\cf{Server.initMessagePassing}$($\fc{f}^{\hopiter-1}_\theta$, $m$)

    \textit{// Clients share embeddings with their neighbors}
    \STATE $\cf{AsyncMessagePassing}$(Clients, $timeout$, $\hopiter$)
    \ENDIF
    \STATE $\fc{f}^{\hopiter}_\theta$ = $\cf{FederatedLearning}$(Server, Clients, $\hopiter$, $R$)
\ENDFOR
\STATE {\bfseries Output:}{Trained \toolgnn $\fc{f}_{\theta}$}
\end{algorithmic}
\end{algorithm}

==> appendices/communication.tex <==
\section{Communication Cost}
\label{appdx:comm}

\subsection{GNN}
In a typical message-passing GNN all the layers of the model are trained together. As a result, in a single epoch, each train and validation client requires the features and intermediate embeddings of its neighbors and need to send back gradients to them. Only the features of the neighbors can be cached by a client as rest of it keeps changing in every epoch. In each training round, only a small set of clients get the model from the server for training and validation tasks. Therefore, the clients in the $\num$-hop of neighborhood of these clients need the model too. Server being unacquainted by the neighborhood of any client, an efficient way to provide models to the neighborhood of train and validation clients is through train-clients only. So, in every round, a client upon receiving the model from the server, either for training or validation, propagates it in its $\num$ hop neighborhood. Eventually, sending and receiving models, embeddings and gradients contribute to the client-to-client communication of training GNNs in federated setup. Client-to-server communication include the cost to receive the model in a round for training and send back the gradients to aggregate.

\subsection{\toolgnn }
Following the training procedure for \toolgnn as described in \ref{sec:retexo-train}. Each train and validation node requires embeddings from the previously trained model. It might be the case that the node selected for a round or any other node in its $\num$ hop neighborhood doesn't has the previously trained model. To avoid such situation, server performs a sync i.e. send the trained model after finishing training for each model in \toolgnn to every node. Such a sync is unreasonable for layers in case of GNNs as it will increase the communication cost significantly. Similar to the features in the case of GNNs, In \tool every node can cache the embeddings of its neighbors after every model as it will remain same throughout the training process. In our implementation, after the sync from the server, each compute its embeddings on the latest model and share it among all it neighbors before the start of the training of next model. Finally, only sharing of embeddings after every model except last contribute to the client-to-client communication of training \toolgnn in federated setup. For client-to-server channel, it includes the cost to receive models and send back gradients in a round and some additional cost to sync the latest trained model after training each model. Still the total cost over client-to-server is significantly lesser than in case of GNNs because of the reduced size of models in \toolgnn.

==> appendices/gcn-train.tex <==
\section{Distributed \gcn Learning}
\label{appdx:gcn-learning}

In each training round, the server sub-samples a set of nodes from all available train-clients and assigns training and validation tasks to them. For training a $2$-layer \gcn, here we detail the actions performed during the message-passing round by the client that received the training task.

% \server The server distributes the model parameters $\fc{f}_\theta$ to the train-clients ($\Gamma[\set{V}]\subset \set{V}$) that are ready to participate in that round of training. 

\subsection{Message Passing}
\paragraph{First representations} The train-client $v$ sends its first representation $\arr{Q}^0_v$ and the \gcn's first layer $\theta^0_{IH}$ to its neighbors $u\in \set{N}(v)$. The neighbors of the train-client will do two things. First, they will reply to the train-client with their own first representation $\arr{Q}^0_u$. Second, they will request their neighbors to share their first representations with them so that they can compute their second representation $\arr{Q}^1_u$. The $2$-hop neighbors of the train-client will then reply with their first representations.

\paragraph{Second representations} Once the train-client and its neighbors receive the necessary first representations, they will start computing their second representation using the model.

\begin{align*}
\arr{Q}^1_v &= \sigma(\frac{1}{\cf{deg}(v)}\cdot \sum_{u}\arr{Q}^{0}_u\cdot\arr{\theta}^0_{IH})\\
\arr{Q}^1_u &= \sigma(\frac{1}{\cf{deg}(u)}\cdot \sum_{u'}\arr{Q}^{0}_{u'}\cdot\arr{\theta}^0_{IH})\text{, } u'\in\set{N}(u)\text{, }u\in \set{N}(v)
\end{align*}

The train-client's neighbors will send their second representations to the train-client. The train-client can then compute the final representation, i.e., the node embeddings. 

\begin{align*}
    \arr{Q}^2_v = \sigma(\frac{1}{\cf{deg}(v)}\cdot \sum_{u}\arr{Q}^{1}_u\cdot\arr{\theta}^1_{HO})
\end{align*}

% training clients sends its second representation to its neighbors and asks its neighbors to respond with their own second representations. However, notice that the neighbors of the training client have to ask their neighbors to send them their first representations to compute their own second representation. So, they ask their neighbors ($2$-hop neighbors of training clients $v$) to send them their first representations. The neighbors of the training clients then compute their second representation.

Similarly, if the \gcn had $\num$-layers then all the nodes in the $\num$-hop neighborhood will participate in the message passing. The nodes at a distance of $p$ will compute $0^{th}$ to ${\num-p}$ representations.

\subsection{Gradient Computation}

\client Each training client $v$ will compute the loss and gradients with respect to the parameters. However, notice that the weights are shared between the nodes and their neighbors. For the shared parameters, the gradient computation would require additional factors, i.e., a real-valued array representing neighbor's input to the shared weights during the forward pass, from the neighbors. A train-client will have to ask its neighbors to provide the necessary factors. Therefore, the gradients can only be computed with another round of message passing. The factors are dependent on the model architecture. In a \gcn, the first layer parameters are shared. Therefore, for each neighbor of the train-client, it will have to ask the input to that layer used by its neighbor during the forward pass. Therefore, the size of factors required from a neighbor is the size of the input to that layer. For a $\num$-layer \gcn, these factors would come from $(\num-1)$-hop neighbors. The message passing is conducted similar to the one during the forward pass.

% At the end of the message passing, each train-client will update the model based on a pre-decided learning rate and send their local models to the server. The server will aggregate the local models and use it to start the next round.

\subsection{Model Aggregation}

Each sampled train-client ($v$) will locally update the model based with learning rate $\eta$.

 \begin{align*}
     \fc{f}'_{\theta}[v] = \fc{f}_{\theta}[v] - \eta\cdot\frac{\partial L_{v}}{\partial \theta}
 \end{align*}

All sampled clients for training share their updated model with the server. The server will aggregate the locally updated models and use it to start the next round.

% \server The server will receive all updated models which then computes the aggregated model. The server will share this aggregated model in the next round of the learning process.

% \begin{align*}
%     \fc{f}'_{\theta} = \sum_{v}{\fc{f}'_{\theta}[v]}\text{, }v\in\Gamma{\set{V}}
% \end{align*}

==> appendices/tool-train.tex <==
\section{Training \toolgnn}
\label{appdx:tooltrain}

\input{algorithms/fl.tex}
\input{algorithms/messagep.tex}


We provide more detailed algorithms for federated learning and message-passing rounds to train \toolgnns in Algorithms~\ref{alg:fl} and~\ref{alg:messagep} respectively.

\subsection{Federated Learning}
\label{appdx:toolfl}

We use the $\cf{FedSGD}$ protocol to train every \mlp in \toolgnn. The server knows all the clients, and which ones to use for training, validation, and testing (Line $2$ in Algorithm~\ref{alg:fl}). The clients locally store their own feature vector, label, and their neighbors (Line $3$ in Algorithm~\ref{alg:fl}).  The clients have access to the optimizer used for training too. In practice, the server can send the optimizer, with a fresh internal state, to the clients before training a model. As the training of the model goes by, each client's optimizer's internal state changes locally until the training is completed. Finally, the clients will locally store their neighbors' embeddings from all previous message-passing rounds.

Consider a scenario where the server wants to train the model $\text{\mlp}_m$, i.e., the $m^{th}$ \mlp. The server will first initialize the model (Lines $5$-$6$). For each training round, the server will sample a set of clients, from the set of train-clients, for training and another for validation. The server then sends a message to these clients along with the most recent state of the model and the task that clients have to perform (Lines $8$-$10$). On receiving this message from the server, each client proceeds to execute the requested task (Line $18$). If a client is requested to train the model then the client will perform one forward-pass and one backward-pass on the model. It will update the model based on the learning rate, weight decay and the momentum, as given by the optimizer's internal state. The client will then return the updated local model to the server (Lines $19$-$21$). If a client is requested to validate the model then the client just evaluates the model on its feature vector and lets the server know if the predicted label is correct.

The server waits for the updated local models from the sampled clients. On receiving all of them, the server will proceed to aggregate the models and start a new round of training with that model (Lines $11$-$14$).~\footnote{The $\cf{FedSGD}$ protocol can be modified to handle asynchronous and unreliable networks too~\cite{nguyen2022federated}.} The number of training rounds can be fixed beforehand, based on the budget available, or the training can be stopped early by tracking the validation accuracy.


\subsection{Asynchronous Message Passing}
\label{appdx:mp}

The server initiates a message-passing round before training an \mlp (except for the first one) by sending the latest updated model to all the clients. For instance, if the server wants to train $\text{\mlp}_m$ then it will first send all the clients $\text{\mlp}_{m-1}$ and ask the clients to start the message-passing round. The clients will use its own features, embeddings, neighbors' embeddings from previous message-passing rounds, and previously trained models to compute the current embedding $Q^m$ (Line $5$). The client then shares this embedding with its neighbors (Lines $9$-$14$) when the communication channels are available. For instance, in proximity networks, the sharing happens whenever they are in proximity. In distributed social networks, the sharing happens whenever the neighbors are online and a successful connection with them is established.



==> chapters/abstract.tex <==
Abstract goes here.

==> chapters/acks.tex <==
% \section*{Acknowledgments}
% We thank Crystal Center and its sponsors, Singapore Ministry of Education (MoE), National University of Singapore (NUS), and National Research Foundation Singapore (NRF) for their generous grants. Aashish Kolluri is supported by Crystal Centre under the Grant No.: E-251-00-0105-01 and MoE under the Grant No.: A-0008530-00-00. Bryan Hooi is supported in part by NUS ODPRT grant under the Grant No.: R252-000-A81-133.

==> chapters/approach.tex <==
\section{GNNs for Fully-Distributed Setup}
\label{sec:gnnsdist}

Existing GNNs do not naturally extend to the proposed setup since message-passing is built into the end-to-end training process. We illustrate this using a $2$-layer \gcn.
% \subsection{A Prospective Distributed GCN}
% \paragraph{Graph convolutional network (GCN).} 
%
\gcn is a canonical example of message-passing GNNs with the $\cf{AGGR}$ being a mean function, i.e., a node's representation is an average of its neighbors' representations. For a \gcn, the equation~\ref{eq:1} can be written as follows:
{\small
$$
\arr{Q}^\hopiter_v = \arr{\theta}^{\hopiter-1}\cdot\cf{Concat}(\arr{Q}^{\hopiter-1}_{v}, \cf{Mean}_{u\in\set{N}(v)}(\arr{Q}_{u}^{\hopiter-1})), \hopiter \in \{1,\ldots,\num\}
$$
}
% where $\tilde{\Ac}$ is the degree-normalized adjacency matrix of size $|\set{V}|\times|\set{V}|$, 
% $\arr{Q}^0$ is the input node features with dimension $I$, and $\arr{\theta}^{\hopiter-1}$ are the weight parameters with hidden size $H$.~\footnote{In practice, there is a non-linear activation (ReLU) on every $\theta$.}

% Therefore, 
% A \gcn can be parameterized by its set of weight layers $\{\arr{\theta}^0,\cdots, \arr{\theta}^{\hopiter-1}\}$. 
% To train a \gcn is to learn a function that assigns real values to these weight layers. Typically, \gcn with two layers achieves the best results for node classification. 
% A two layer \gcn can be simply represented as $\{\arr{\theta}^0_{IH}, \arr{\theta}^{1}_{HO}\}$. $\arr{\theta}^0_{IH}$ represents the first layer which transforms the input node features with dimension $I$ to the hidden dimension of size $H$. $\arr{\theta}^{1}_{HO}$ represents the second layer which transforms the hidden features with dimension $H$ to output embedding with dimension $O$.



\subsection{Baseline: Fully Distributed GCNs}
\label{sec:train-gcn}

% width=5.5cm, height=4.8cm
\begin{figure}
    \centering
    \includegraphics[scale=0.40]{figures/message-passing2.pdf}
    \caption{A single train-client $v_i$ performing forward pass with its $1$-hop neighbor $v_j$ and $2$-hop neighbor $v_k$ in one training round.}
    \label{fig:message-passing}
\end{figure}

The training protocol for \gcn in the fully-distributed setup would be as follows: The \gcn is trained across $\numrounds$ training rounds. Each training round begins with the server sending aggregated \gcn layers to the {\em train-clients}, the clients that participate in that training round. The train-clients then perform two message-passing rounds, one each for the forward and the backward pass, wherein they mobilize the clients in their $2$-hop neighborhood.  Figure~\ref{fig:message-passing} shows the message-passing for the forward pass.

In the forward pass, a train-client will send the first layer of the \gcn to its neighbors and ask them for their initial representations, i.e., raw features (see (1) in Figure~\ref{fig:message-passing}).
% ~\footnote{Sending raw features can be avoided by using an additional non-invertible weight layer on the features before aggregation.} 
The $1$-hop neighbors will then ask their neighbors for initial representations. The $2$-hop and $1$-hop neighbors will reply with their initial representations (2). The $1$-hop neighbors will use their neighbors' initial representations and the first layer to compute the hidden representations, which they send to the train-clients (3). The train-clients use their neighbors' initial and hidden representations to compute the output embedding.  

The backward pass would also require another round of message-passing since certain weights are shared by multiple nodes. Concretely, the train-client would have to ask its neighbors for certain factors to compute the gradient, and the neighbors need such factors from theirs too. 

Appendix~\ref{appdx:gcn-learning} gives more details of the training process. One noteworthy design decision we make is that the clients send layer parameters to their neighbors instead of the server. One reason, among others (see Appendix~\ref{appdx:gcn-learning}), is that the server does not know neighbors of any client, and the neighbors querying the server for layers may trivially reveal the edges to the server and other auxiliary private information such as mobility patterns in proximity networks. This also illustrates why, in our setup, we assume that the clients only reveal the gradients to the server. 

\subsection{Problems with Distributed \gcn}
\label{sec:gcnproblems}

\noindent\textbf{Challenge 1.} Training GNNs may require {\em high volume of data transfer}. For instance, the data transferred per client is as follows:

% In each training round, \gcn requires  many rounds of communication between the clients in $\num$-hop neighborhoods. This leads to {\em high latency and data transfer volumes}. For instance, the data transferred per client is as follows:

% \paragraph{P1: Raw data sharing} During message-passing, the clients have to share their raw features ($H^0_v$) with their neighbors in the first round of message-passing. In typical message-passing GNNs, this is the first step. Further, there can be situations where a client's raw features are propagated beyond $1$-hop neighbors. If the graph were a social network, then $2$-hop neighbors might not be trusted by a client. Therefore, a client cannot have control over their raw data if they agree for training such GNNs.   

% In each training round, for each train-client the server sends the updated model
When the degree of a train-client is $d$, the train-client will send the parameters of the first layer to its $d$ neighbors. If $H$ is the number of hidden dimensions, then the size of the first layer will be $2IH$ and the number of parameters sent by the train-clients is $2IHd$. The clients from the $1$-hop neighborhood would receive the layer.  The number of parameters received by such clients would be $2IH$. Across $\numrounds$ rounds of training, the data transferred by the train-clients is about $2IHd \numrounds\times 32$ bits.~\footnote{Assuming the parameters are represented using $32$-bit floating point precision.} Further, the data transferred by each neighbor of the train-clients is $2IH \numrounds\times 32$ bits. 
%
The hidden representations and factors required for gradients would be $O((I+H)d)$ and $O(Id)$ bits respectively.

\textit{Cost Illustration.} Consider a $2$-layer \gcn where $I=1000$ and $H=256$. Let there be a train-client with $d=10$ neighbors. The total data transferred by it during a forward pass for one training round would be $2\times1000\times256\times10\times32 = 160$ Mb. If the model is trained for $R=400$ rounds, the total data transferred just for message-passing during forward pass for that train-client is $64$ Gb. Further, the neighbors of this train-client would transfer at least $6.4$ Gb. These costs are already prohibitive for a simple $2$-layer \gcn. For each train-client and their neighbors, these costs would increase linearly with degree, input size, size of additional pooling layers, and the number of layers $K$.

% For instance, the clients in proximity networks could be mobile phones with low-bandwidth networks.

\noindent\textbf{Challenge 2.} Training GNNs may not be possible when the networks are mobile and asynchronous. Implementing the backward pass requires re-designing the automatic gradient computation for asynchronous networks. This is a challenge in itself and further demands {\em high availability} from the clients.
%
For instance, in proximity networks, the backward pass will fail if the neighbors of a node available during the forward pass are not available for the backward pass. The problem is exacerbated when $2$-hop (and higher order) neighbors are necessary. Even if everyone was available for one round, assuming such availability for all training rounds is not practical. Finally, the real-world implementations of federated learning over mobile devices usually train the models at night when the devices are plugged in to the charging points~\cite{bonawitz2019towards}. GNNs cannot be trained with such constraints in mobile and proximity networks since message-passing is necessary in every training round. 




% \noindent\textit{Latency} If the delay on the communication channels among the clients is $c$ then, for a $\num$-hop GCN, the total delay incurred during the message-passing rounds is $O(\num^2\cdot c)$. Note that this delay is considering that all the non-training clients are also available during a training round which may not be possible in many real-world scenarios. If the clients are unavailable due to network issues or power-saving constraints then the delay could be exacerbated.


% \paragraph{Communication in FL Setup for GCN}
% In the general working of the FL environment the central server shares the global model across the network to all the devices that are participating in a single round of federated learning. The total number of devices that are participating can go really high and the bandwidth over which the devices are connected to the environment could be relatively slow and unstable.

% In an FL training environment, there can be many rounds of communication that exist between the central server and all participating devices. Over a singular communication round the global model is shared across all the devices in the FL environment and each participating device downloads the global model to train it on their local data. A version of that is uploaded back to the environment to the central server. Therefore there is a constant downlink and uplink during the communication rounds. The overall communication cost of sharing model updates.
% We can define few metrics for measuring the efficiency of communication in our setup - 
% \begin{enumerate}
%     \item \textbf{Number of messages exchanged for a particular node (with peers and with server)} - In order to compare the communication efficiency of setup, we can compare the total number of messages exchanged by a single node and the central server. In a single round of federated learning, a node has to receive a aggregated gradient and send the local gradient back to the main server. For a $k$ layers deep GCN, a node has to query its neighbor $k $ times for their embedded representation vectors and another $k $ times for their gradient. So total messages exchanged for a node in a single round will sum up to 2 gradients with the central server, $k$ gradients with every neighbor and $k$ embedded representation vector with every neighbor. For the server, it has to receive gradients from all participating nodes in that round.
%     \item \textbf{Size of messages exchanged} - In addition to the number of messages exchanged, total size of messages exchanges is also a good metric to compare the communication efficiency. If the number of parameters in our GCN is $p$, every node has to share gradients corresponding to each parameter with the central server and with the neighbors. In a single round of federated learning, a nodes sends and receives $p \times d \times32$ bits among the neighbors where $d  $ is the degree of the node and $p \times 32$ bits with the central server for sharing gradients only. Along with this, a node sends $f \times d \times 32$ bits, here $f $ is the total number of features including initial, hidden and outputs features of our GCN and $d $ is the degree of the node. So the total size of messages shared on peer to peer channel is about $2 \times(p\times d \ + f\times d)\times 32$ bits and the total size of messages between central server and a node is about $2 \times p \times 32$ bits.
%     Now, if lets say $p = 10^5$, $f = 5 \times 10^3$ and $d = 20$, then a node has to send and receive $67.2$ Mb of data with the peers and $3.2 $ Mb of data with the server. The central server has to send and receive $3.2 \times c$ Mb of data where $c $ is the number of nodes participating a particular round of federated learning.
%     \item \textbf{Number of nodes participating in a single round of FL} - This metric is more concerned about the central server. The data exchanged with the central server will be directly proportional to the number of nodes participating in a particular round. Due to limited capacity of central server and bandwidth, the size of messages exchanged with the central server by a single node can limit the number of participants of each round given we have to finish it within some constant time.
% \end{enumerate}


% \subsection{\tool Architecture}
% This section is to describe the federated learning protocol which is being used by the framework to extend any typical GNN. The participants in the protocol are nodes having attributes and edges and a centralized FL server. In each iteration of the protocol, multiple nodes participate in the learning and train their local MLPs, till the shared model converges over multiple round of federated learning, on their data and aggregate their embeddings with the neighbors after that . A round in federated learning is completed as follows :

% \begin{enumerate}
%     \item The central server randomly initialize the parameters of the shared model and sends its parameters to the nodes before the training of the local models in the node begins.
%     \item Nodes start to train their local models over their own data by using these parameters.
%     \item Each node updates its parameters while training its own model. Each node computes one-step gradient which for node $k  $ in round $t $ can be $g_t^{k(1)}=\nabla_{\omega_t} \mathcal{L}_k\left(\omega_t ; \mathcal{D}_k\right)$ where $\mathcal{D}_k$ is the data on the node $k$ , $\omega_k$ is the model parameters at the start of round $k$, and $\mathcal{L}_k$ is the loss function.
%     \item Next, the central server gathers all the gradients and applies the update with average $$ \omega_{t+1} \leftarrow \omega_t-\eta \sum_{k \in K} \frac{g_t^{k(1)}}{|K|}$$ where $K $ is the nodes participating in this round and $\eta$ is the learning rate. 
% \end{enumerate}
% After all the nodes end up training their MLPs in this setup (after multiple FL Learning rounds), every node aggregate the embedded representation vectors with the neighboring nodes using the aggregate method of the base GNN as 
% $$\mathbf{z}_{\mathcal{N}(k)}^{i - 1} \leftarrow \operatorname{AGGREGATE}_i(\{\mathbf{z}_v^{i-1}, \forall v \in \mathcal{N}(k)\})$$
% $$\mathbf{f}_{k}^{i} \leftarrow \operatorname{CONCAT}(\{\mathbf{z}_v^{i-1}, \mathbf{z}_{\mathcal{N}(k)}^{i - 1}\})$$
% where $z_v^i$ is the embedded representation vector of each node after $i $ iterations of protocol, $\mathcal{N}(k)$ denotes the neighbour of node, $\mathbf{z}_{\mathcal{N}(k)}^{i - 1}$ represent the aggregated embedded vector representations of neighbors of node $k$  and $\mathbf{f}_k^i$ represent the initial features for $ith$ iteration.Then, each node use the aggregated embedded vector representation for another iteration of training MLPs. And we claim that the results after multiple iterations of this sort are comparable



==> chapters/arch.tex <==
\section{The \toolgnn Architecture}
\label{sec:arch}

% What is the key idea?
% \bryan{This part should be an overview, where you give the overall motivation / benefits / design ideas (something like the current 1st 2 paragraphs). The subsequent paragraphs seem like too much detail, the precise explanations should be in the subsections. }

We present a novel graph learning architecture called \tool to address the aforementioned challenges. \tool can be seen as a generic transformation of a traditional GNN into its \tool counterpart that retains the  $\cf{AGGR}$ and $\cf{COMBINE}$ functions in the original GNNs. 

% This is important for preserving the design principles of the GNN which in turn preserves accuracy in homophilous, heterophilous~\cite{zheng2022graph}, and inductive settings~\cite{hamilton2017inductive}.

In GNNs, the edge structure is sandwiched in between the trainable layers. Therefore, all layers' parameters are optimized simultaneously using message-passing in each training round.
% In a fully-distributed setup, this is expensive as it requires syncing parameter state between neighbors in a training round. 
\tool remedies the GNN architecture by {\em decoupling} the edge structure from the training of layers and delaying the message-passing to only {\em after} the training of one layer completes. For instance, if a \gcn has $2$ layers then the \tool framework will deconstruct the $2$ layers, turn each layer into a classifier without the edge structure, and train them sequentially one after another. After training each classifier, the $\cf{AGGR}$ and $\cf{COMBINE}$ functions are applied to the logits corresponding to the previous classifier. Specifically, for \toolgcn, the nodes compute the mean of their neighbors' logits and concatenate that with their own logits. The resulting logit array is used as features to train the next classifier. The classifier could be any trainable neural network, however, we just choose an \mlp.

% Encapsulating both the ideas, we design the \tool framework that advocates a novel design principle for the fully-distributed setup. Instead of training a GNN end-to-end the idea is to train the GNN layer by layer. The message-passing phase is only conducted after completely training every layer, therefore, a GNN is effectively unrolled. 

Therefore, while training a \toolgnn, the message-passing rounds are independent of the training rounds of each \mlp. This drastically reduces the number of message-passing rounds from $O(R)$ to $\num$ which further reduces the total data transferred over the network. Computing gradients while training the layers does not require any message-passing since each \mlp is trained independent of the graph structure. This makes training practical on mobile and asynchronous networks.

% Furthermore, \tool naturally extends to the federated setup wherein a large sub-graph is stored at every client instead of a single node. Therefore, \tool remains compatible with training improvements developed for the federated learning setup as well. Examples of such improvements include federated optimization~\cite{reddi2020adaptive}, handling for asynchronous real-world deployments~\cite{bonawitz2019towards,nguyen2022federated}, defenses against data poisoning, and training for better robustness~\cite{liu2022federated}. 

\subsection{Architecture of \toolgnns}

% \prateek{I don't think \tool is a "tool that transforms GNN to RetexoGNN", though you make it sound like that. It's a conceptual transformation: a mapping technique. I suggest we be very clear about this and not misinform.}

For a $\num$-layer base GNN, the \toolgnn counterpart is a collection of  $\num+1$ independent \mlps (see Figure~\ref{fig:tool}). 
% The additional model is to avoid sharing raw features directly with neighbors.
%
The first \mlp is used to learn embeddings from the node features. There are $\num$ more \mlps after the first one, each having the $\cf{AGGR}$ and $\cf{COMBINE}$ layers of the base GNN. The first \mlp can be avoided in \toolgnns if the raw features can be shared with neighbors similar to GNNs. \toolgnn's intermediate embeddings (logits after every model) are given by:
{\small
\begin{align*}
    \arr{Q}^{\hopiter}_v &= \fc{f}^{\hopiter-1}_\theta(\cf{COMBINE}(\arr{Q}^{\hopiter-1}_v, \cf{AGGR}^{m-1}_{ u\in\set{N}(v)}(\arr{Q}^{\hopiter-1}_u))),\\
    &\hopiter\in\{2,\ldots, \num+1\}\text{;  } \arr{Q}^{1}_v = \fc{f}^{0}_\theta(\arr{Q}^0_v)\\
\fc{f}^{\hopiter-1}_\theta &= \text{ \mlp}_{m-1} = (\arr{\theta}^{\hopiter-1}_{OH}, \arr{\theta}^{\hopiter-1}_{HO}),\\
&\hopiter\in\{2,\ldots, \num+1\}\text{;  } \fc{f}^{0}_\theta = \text{ \mlp}_{0} = (\arr{\theta}^{0}_{IH}, \arr{\theta}^{0}_{HO})
\end{align*}
}%

For $(\arr{\theta}^{\hopiter-1}_{OH}, \arr{\theta}^{\hopiter-1}_{HO})$ above, the $\arr{\theta}_{OH}^{\hopiter-1}$ converts the aggregated embeddings to a representation of size $H$ and the $\arr{\theta}^{\hopiter-1}_{HO}$ converts that into the output. In our running example, the $2$-layer \toolgcn can be represented by $\{\text{\mlp}_0:(\arr{\theta}^{0}_{IH}, \arr{\theta}^{0}_{HO}),\text{ \mlp}_1:(\arr{\theta}^{1}_{OH}, \arr{\theta}^{1}_{HO}),\text{ \mlp}_2:(\arr{\theta}^{2}_{OH}, \arr{\theta}^{2}_{HO})\}$. 


\begin{figure}
    \centering
    \includegraphics[scale=0.21]{figures/retexo.pdf}
    \caption{Base GNN to its \toolgnn.}
    \label{fig:tool}
\end{figure}

\subsection{Training a \toolgnn}
\label{sec:retexo-train}
For training every \mlp we use the traditional federated learning approaches. Before training each \mlp, except the first one, we do a message-passing round to get the embeddings from a node's neighbors. We describe an outline of the training protocol here (see Algorithm~\ref{alg:outline}) and provide full details, for the federated learning and message-passing protocols in the Appendix~\ref{appdx:tooltrain}.

\paragraph{Federated Learning.}
The server and the clients together train $\num+1$ models sequentially. For each model, the training proceeds in rounds. The server samples a subset of the train-clients for each round and delegates training / validation tasks to them. In each training task, the server shares the model parameters with the selected clients.  The clients perform a forward and backward pass on the model using their local data and return the updated local model to the server. In each validation task, the server just asks the clients to report their accuracy. Notice that to compute the $\cf{AGGR}$ layer, the client uses the embeddings collected from its neighbors in the previous message-passing round. Each client has a single input (feature vector and a label). Hence, it carries out only a single forward and backward pass per training round. Therefore, this is equivalent to the standard FedSGD training protocol. For the federated setup with multiple nodes per client, the FedAVG protocol could be used wherein multiple forward and backward passes are carried out locally~\cite{mcmahan2017communication}.
%
% After training each \mlp for $\numrounds$ rounds, we do one round of message-passing between the clients.
%A key difference between the traditional federated setup for images and our current setup is that there is every node has only one data point and one label associated with it.

\paragraph{Message-Passing.}
Before training the $\hopiter^{th}$ \mlp, the server initializes a message-passing round by sending all the clients the $(\hopiter -1)$ trained \mlp parameters, i.e., it syncs the latest model with the clients. The clients then compute embeddings from it and share them with their neighbors. For example, consider a \toolgnn with three \mlps and say the server is training its third \mlp. At this point, the server sends the second model to all clients. So, now all clients will have the first \mlp ($\text{\mlp}_0$), their own first embeddings output by their first \mlp ($\arr{Q}_v^1$), the first embeddings obtained from their neighbors ($\arr{Q}_u^1$, $u\in\set{N}(v)$) from the previous message-passing round, and the second \mlp ($\text{\mlp}_1$). The clients locally compute $\arr{Q}_v^2$ using this information. The clients then share $\arr{Q}_v^2$ with their neighbors to complete the current message-passing round. In highly asynchronous networks, one successful message-passing round, including the sync, can take up to many hours or days. This underscores the importance of having only a few message-passing rounds, such as in \tool.

\paragraph{\tool Features.} The architecture and training protocol of \toolgnns ensure that the privacy constraints (see Section~\ref{sec:main_problem}) are satisfied. First, only the locally-trained model parameters are shared with the server, which can further be protected if necessary using secure aggregation~\cite{bonawitz2017practical} for instance. Second, the logits (or raw features) will be shared {\em only} with the neighbors and are not propagated further before applying an irreversible function (due to the non-linear ReLU activations). \toolgnn's layers (\mlps) could be trained as long as the client-to-server communication channels are available, for instance, on plugged-in mobile devices at night. After training each layer, the message-passing can be performed independently when the client-to-client channels are available, for instance, when mobile devices are carried around during the day. Only the small embeddings have to be shared on client-to-client communication channels, which can be quickly done even in low-bandwidth proximity networks. The order in which messages are exchanged does not matter either. Further, all neighbors of a client do not need to be available for a message-passing round; the client can aggregate embeddings received from the available nodes. \tool is robust to such unavailability. Experiments reported in Appendix~\ref{appdx:robustness} elaborate on this feature of \toolgnns.

Finally, \tool naturally extends to the federated setup, wherein a large sub-graph is stored at every client. Therefore, \tool remains compatible with training improvements developed for the federated learning setup, for instance, federated optimization~\cite{reddi2020adaptive}, handling for asynchronous real-world deployments~\cite{bonawitz2019towards,nguyen2022federated}, defenses against data poisoning, and training for better robustness~\cite{liu2022federated}. 



% We emphasize that, unlike in a GNN, training \toolgnn would require clients to share only the embeddings and only once per message-passing round which is practical even in weak mobile network environments. Further, having only $\num$ rounds of message-passing makes it feasible for the server to sync the model with all the clients after training it. 



\input{algorithms/outline.tex}

% \subsection{\toolgcn vs GCN}


% We will show the improvements in communication efficiency more concretely. First, for a $2$-layer \toolgcn, the total data transferred per train-client during message-passing phase $d\cdot(|\text{\mlp}_0|+|\text{\mlp}_1|) = d\cdot(IH + HO + 2OH+HO)$. Therefore during message-passing, \toolgcn requires $\numrounds$ times lesser data to be transferred than the \gcn across all rounds. If we take the communication with the server also into account, then in \toolgcn, the train-clients transfer $d$ times less data than in \gcn and the test-clients in the neighborhood of the train-clients will transfer $\numrounds$ times less data than in \gcn.

% In fact, we prove the following general theorem that is true for most message-passing GNNs.

% \prateek{A theorem?}
% \begin{theorem} Consider any GNN with structure described in Section~\ref{} where $\cf{AGGR}$ function uses a linear layer with output dimension $P$, $I\geq5O$, $H\geq2O$, $P\geq H$. If both the GNN and the \toolgnn are trained for $R$ rounds then the \toolgnn would require at least $d$ times less data transferred by the train-clients and $R$ times less data transferred by the test-clients from the $\num$-hop neighborhood.
% \end{theorem}



% \subsection{Privacy-Preserving Protocols Integration}
% Without additional privacy protection, \toolgnns may be susceptible to reveal the features and likely the edges from the local models shared with the server during training. However, one can integrate \toolgnn with heuristic defenses such as gradient pruning, and concrete defenses such as secure multi-party computation and differential privacy mechanisms in to its training. We leave extending \toolgnn to support these mechanisms for future work.

% Further, a recently proposed architecture called LPGNet is a special case of \tool framework.





% Concrete End-to-End training procedure, Inference in appendix

% How Retexo deals with the issues mentioned in the previous section

% Adding of existing privacy mechanisms



==> chapters/eval.tex <==
\section{Evaluation}
\label{sec:eval}
We evaluate \toolgnns on $3$ aspects: 

\noindent \textbf{a) Utility.} How do \toolgnns perform in the transductive, inductive, and heterophilous settings?\\
\noindent \textbf{b) Communication-efficiency.} How would \toolgnns communication costs compare to those of the baseline GNNs if they were to be trained in the fully distributed setup? \\
\noindent \textbf{c) Feasibility.} Are \toolgnns currently trainable end-to-end on mobile clients? 

% \noindent \textbf{Robustness to missing neighbors.} How robust are \toolgnns to missing neighbors during message-passing?

\subsection{Experimental Setup}
\label{sec:expsetup}
We consider three widely-used traditional GNNs that are known to perform well across most settings: \gcn~\cite{kipf2016semi}, \sage~\cite{hamilton2017inductive} with max-pooling aggregation layers, and \gat~\cite{velivckovic2017graph}.~\footnote{We use simple mean aggregation instead of localized spectral convolution for GCN as described in~\cite{hamilton2017inductive}.} 

% We implement GNNs with $2$ aggregation layers and for \sage, we use the max-pooling layer for aggregation.

We report the node classification accuracy for utility. For communication-efficiency, we measure the total number of bytes that would be communicated over the network to train the neural networks. Finally, to demonstrate the feasibility of training RetexoGNNs on mobile embedded systems, we use Raspberry Pi boards (RPi) as clients. It is hard to demonstrate the fully-distributed setup since we would need a large number of RPis. Instead, we use $2$ RPis and horizontally split the graph data to store on the RPis. We train RetexoGNNs with these two clients and a server. The RPis communicate with the server over the internet and with each other over Bluetooth when in proximity. Quantitatively, we measure the total training time and the amount of communication done over the internet and Bluetooth. Qualitatively, we discuss what steps are involved in performing such training and how this would extend to the fully-distributed setup. We report the quantitative results in Section~\ref{sec:results}. We detail the full experimental setup and the qualitative analysis in the Appendix~\ref{appdx:feasibility}.

\noindent{\bfseries Datasets.}
We consider $5$ popular datasets including $3$ citation and $2$ social networks
%and $2$ large OGB datasets 
for the homophilous-transductive setting~\cite{wu2020comprehensive,hu2020open}. For the heterophilous-transductive setting, we evaluate on $2$ datasets \wikicooc and \romane that have been recently introduced~\cite{platonov2023a}. We change the architecture of our three base GNNs as specified in that paper for the heterophilous datasets. For the inductive setting, we construct evolving graphs similar to prior work, from the homophilous-transductive datasets~\cite{zeng2019graphsaint}. We provide full details on the datasets and architectures in Appendix~\ref{appdx:datasets}.

\noindent{\bfseries Implementation \& Training.} To emulate practical implementations of federated learning protocols, we diverge from the traditional epoch-based training in the centralized setup to round-based~\cite{bonawitz2019towards}. In each round, we randomly sample a batch of train nodes and validation nodes, up to $1024$ total, independent of the previous rounds. 
% We sample the neighbors considered for aggregation up to a maximum of $25$ across every hop, as in~\cite{hamilton2017inductive,platonov2023a} 
We fix the total number of rounds to $400$ in the transductive and inductive settings whereas $1000$ in the heterophilous setting. 
%
We also separately implement early-stopping to measure the communication costs required to just reach convergence. It is difficult to identify a common criteria for early-stopping across all evaluated configurations. So, we manually chose the patience as $30$ since that is much smaller than $400$ and gave us the best results for GNNs in most configurations.
%
We provide more implementation details in the Appendix~\ref{appdx:impl}.


% \begin{figure}
%   \centering
%   \begin{tikzpicture}
%     \begin{axis}[
%       xlabel=Communication (log),
%       ylabel=Accuracy,
%       error bars/y dir=both, 
%       error bars/y explicit,
%       legend style={at={(0.5,-0.2)},anchor=north},
%       legend columns=-1,
%       xmin=500000,
%       % xmax=11000000,
%       xtick={500000,1000000,5000000,10000000},
%       xmode=log,
%       ]
%       \addplot[scatter, only marks, scatter src=explicit symbolic, scatter/classes={
%         gcn={mark=square*,blue},
%         toolgcn={mark=triangle*,blue},
%         sage={mark=square*,red},
%         toolsage={mark=triangle*,red},
%         gat={mark=square*,black},
%         toolgat={mark=triangle*,black}
%         }] table[x=communication,y=acc_mean, y error=acc_std,col sep=comma, meta=architecture]{figures/cora_acc_comm.csv};
%       \legend{\gcn,\toolgcn,\sage,\toolsage,\gat,\toolgat}
%     \end{axis}
%   \end{tikzpicture}
%   \caption{Accuracy vs. Communication}
%   \label{fig:scatterplot}
% \end{figure}


 
 

\input{figures/plot_acc_vs_comm_1}
% \input{communication_costs/cora/plot_cora.tex}






% \begin{table}[t]
% \caption{Micro-F1 scores for node classification in the inductive setting.}
% \label{tab:indresults}
% % \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|l|l|l|l|l}
% Method     & \cora            & \seer        & \pubmed          & \fbpage  & \lastfm    \\ \hline
% \mlp        & $0.64$ $\pm$  $0.01$ & $0.65$ $\pm$  $0.01$ & $0.78$ $\pm$  $0.01$ & $0.71$ $\pm$  $0.01$ & $0.64$ $\pm$  $0.01$ \\
% \gcn        & $0.75$ $\pm$  $0.02$ & $0.69$ $\pm$  $0.02$ & $0.83$ $\pm$  $0.01$ & $0.85$ $\pm$  $0.01$ & $0.76$ $\pm$  $0.01$ \\
% \toolgcn  & $0.67$ $\pm$  $0.02$ & $0.67$ $\pm$  $0.02$ & $0.81$ $\pm$  $0.01$ & $0.81$ $\pm$  $0.01$ & $0.71$ $\pm$  $0.01$ \\
% \sage  & $0.71$ $\pm$  $0.02$ & $0.68$ $\pm$  $0.02$ & $0.82$ $\pm$  $0.01$ & $0.88$ $\pm$  $0.01$ & $0.76$ $\pm$  $0.01$ \\
% \toolsage & $0.72$ $\pm$  $0.02$ & $0.66$ $\pm$  $0.03$ & $0.81$ $\pm$  $0.01$ & $0.84$ $\pm$  $0.01$ & $0.74$ $\pm$ $0.01$ \\
% \gat        & $0.77$ $\pm$  $0.02$ & $0.68$ $\pm$  $0.02$ & $0.81$ $\pm$  $0.01$ & $0.83$ $\pm$  $0.02$ & $0.74$ $\pm$  $0.01$ \\
% \toolgat  & $0.74$ $\pm$  $0.03$ & $0.68$ $\pm$  $0.02$ & $0.81$ $\pm$  $0.01$ & $0.86$ $\pm$  $0.01$ & $0.77$ $\pm$  $0.01$
% \end{tabular}
% }
% \end{table}



\subsection{Results}
\label{sec:results}


\begin{table}[t]
\caption{Micro-F1 scores on heterophilous-transductive datasets.}
\label{tab:transresultsmini}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{l|l|l}
Method    & \wikicooc  & \romane \\ \hline
\mlp       & $0.77$ $\pm$ $0.03$ & $0.65$ $\pm$ $0.00$\\\hline
\gcn       & $0.90$ $\pm$ $0.00$ & $0.75$ $\pm$ $0.00$\\
\toolgcn & $0.87$ $\pm$ $0.00$ & $0.80$ $\pm$ $0.00$\\\hline
\sage  & $0.91$ $\pm$ $0.01$ & $0.82$ $\pm$ $0.00$\\
\toolsage & $0.87$ $\pm$ $0.01$ & $0.84$  $\pm$ $0.00$\\\hline
\gat  & $0.90$ $\pm$ $0.01$ & $0.80$ $\pm$ $0.00$\\
\toolgat  & $0.89$ $\pm$ $0.01$ & $0.82$ $\pm$ $0.00$
\end{tabular}
}
\end{table}

\paragraph{Q1: Node-classification performance.} We present the micro-F1 scores of homophilous-transductive datasets in Figure~\ref{fig:acc_vs_comm} (Y-axis) and heterophilous-transductive datasets in Table~\ref{tab:transresultsmini}. 
%
We present the exact results for the datasets for all transductive and inductive settings in Appendix~\ref{appdx:eval}
% , Tables~\ref{tab:transresults} and~\ref{tab:indresults} respectively. 
Across all evaluated configurations, the performance of \toolgnns is within {\em $2.09\%$} of their respective GNNs on average. \toolgat performs the best among the \tool models across all but one of the evaluated configurations. It sometimes {\em outperforms} \gat in the inductive setting (up to $3.3\%$). In the heterophilous setting, \toolgnns perform better than their respective GNNs by up to $5\%$. 
%\toolgcn is the weakest performing model with $5\%$ less accuracy than the \gcn in $3$ homophilous-transductive datasets.
%
Overall, it is reasonable to expect that \toolgnns will sometimes have worse performance than the GNNs since the aggregation is done over the embeddings of the first \mlp in \toolgnns, unlike in GNNs which aggregate over the raw features directly.



\noindent{\bfseries Q2: Communication-efficiency.}  We report results for communication-efficiency on $5$ homophilous-transductive datasets for the best accuracy ($400$ training rounds) and early stopping settings. In Figure~\ref{fig:acc_vs_comm}, we report the accuracy vs  communication-efficiency comparison for best accuracy setting. We refer to Appendix~\ref{appdx:eval} for all the exact communication-efficiency results.

Training \toolgnns requires $\textbf{3.5}$-$\textbf{18}\times$ and $\textbf{7.77}\times$ on average less data to be communicated over the network than their respective GNNs in the best accuracy setting. Even with early-stopping \toolgnns require $\textbf{2.16}$-$\textbf{43.65}\times$ and $\textbf{12.64}\times$ on average less data than their respective GNNs. Finally, on the possibly unreliable client-to-client communication channels the total data transferred in \toolgnns is \textbf{up to $4$ to $7$ orders of magnitude less} compared to GNNs across all evaluated configurations (see Appendix~\ref{appdx:eval}). This is expected due to the large model layers being communicated on these channels in GNNs (see Section~\ref{sec:train-gcn}). We illustrate our results on the \cora dataset.

Consider \sage and \toolsage which performs $2\%$ worse than \sage in the best accuracy setting. The total data transferred by all clients on both channels is about $10^7$ MB for \sage and about $1.1\times10^6$ for \toolsage which is about $10\times$ lower. 
% Further, the total data transferred on the client-to-client channels for \toolsage is merely $1.13$ MB whereas for \sage it is about $7.7\times10^6$ MB which is $10^6\times$ higher. 
%
% The aforementioned communication-efficiency results are generous towards GNNs. 
As GNNs become deeper, the difference in communication costs between GNNs and \toolgnns will only increase.

\noindent{\bfseries Q3: Feasibility on Mobile Networks.} Unlike GNNs, we show that \toolgnns are practical to train on mobile networks. We implement \tool on the Flower framework~\cite{beutel2020flower}.\footnote{\url{https://github.com/adap/flower}} 
The framework provides client-to-server channels for federated learning. 
We implement our own client-to-client communication channels over Bluetooth. Therefore, when in proximity, the RPis can exchange the logits over Bluetooth. We provide a more qualitative description of our system in Appendix~\ref{appdx:feasibility}.

Quantitatively, we report results for training \toolsage on \cora dataset, which is split in half between two RPis. The total data communicated on client-to-server communication channels, including the headers added by the network protocols, to train the first MLP is $573.04$ MB. For the subsequent two MLPs it is $5.91$ MB each. In total, $0.08$ MB is communicated over Bluetooth for each message-passing round. The maximum RAM consumed on each RPi is $165.44$ MB. The first \mlp takes $463.75$ seconds to train, and the subsequent two \mlps take $49.56$ and $59.68$ seconds respectively. For each round of message-passing \tool requires $63.28$ seconds, which includes the connection time, requesting specific nodes' logits, and exchanging the requested logits. Overall, the RAM consumed is well within the constraints of typical embedded systems ($<1$ GB RAM). 
% and the training time for each model is small as is the time spent on client-to-client communication.

Finally, resource-wise, training \toolgnns is even more practical in the fully-distributed setup since each RPi will consume much less RAM and communicate much less data. For instance, two RPis require only $0.6$ seconds to connect and exchange a single node's embedding. This conclusion is independent of graph size since the resources needed per RPi do not scale with the number of nodes.

% or the number of edges per node since the edges are sampled.

% The total time taken to train a single MLP will not significantly change even in the fully-distributed setup. 
% However, the end-to-end training time may vary depending on how much time is allocated to the message-passing rounds based on the expected mobility patterns. 



==> communication_costs/citeseer/plot_cite.tex <==
\begin{figure}[t]
    \begin{tikzpicture}
        \begin{groupplot}[group style = {group size = 2 by 3, horizontal sep = 25pt, vertical sep = 35pt, xlabels at=edge bottom, ylabels at=edge bottom},
                width=1/3.5*\textwidth,
                height = 3.8cm,
                xlabel={Client},
                x label style={font=\small},
                y label style={font=\small}]
            \input{communication_costs/citeseer/plot_gcn_400.tex}
            \input{communication_costs/citeseer/plot_gcn_es.tex}
            \input{communication_costs/citeseer/plot_sage_400.tex}
            \input{communication_costs/citeseer/plot_sage_es.tex}
            \input{communication_costs/citeseer/plot_gat_400.tex}
            \input{communication_costs/citeseer/plot_gat_es.tex}
        \end{groupplot}
        \node at ($(group c1r3) + (2.05cm,-2.4cm)$) {\ref{grouplegend1}};
    \end{tikzpicture}
    \caption{Comparison of data volume transferred for \seer, $400$ rounds on the left and with early stopping on the right.}
    \label{fig:comm_seer}
\end{figure}




==> communication_costs/citeseer/plot_gat_400.tex <==
\nextgroupplot[title = {\gat vs \toolgat},
    title style={font=\small},
    ylabel={Data transferred in MB}
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/citeseer/gat_400.csv} \closedcycle;
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/citeseer/mmlp_gat_400.csv} \closedcycle;

==> communication_costs/citeseer/plot_gat_es.tex <==
\nextgroupplot[title = {with early stopping },
    title style={font=\small},
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/citeseer/gat_es.csv} \closedcycle;
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/citeseer/mmlp_gat_es.csv} \closedcycle;

==> communication_costs/citeseer/plot_gcn_400.tex <==

\nextgroupplot[title = {\gcn vs \toolgcn},
    title style={font=\small},
    x tick style={font=\Huge},
    legend style={column sep = 1pt, legend columns = 2, legend to name = grouplegend1, font=\small},
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/citeseer/gcn_400.csv} \closedcycle;
    \addlegendentry{GNN}
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/citeseer/mmlp_gcn_400.csv} \closedcycle;
    \addlegendentry{\toolgnn}

==> communication_costs/citeseer/plot_gcn_es.tex <==
\nextgroupplot[title = {with early stopping },
    title style={font=\small},
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/citeseer/gcn_es.csv} \closedcycle;
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/citeseer/mmlp_gcn_es.csv} \closedcycle;

==> communication_costs/citeseer/plot_sage_400.tex <==
\nextgroupplot[
    title = {\sage vs \toolsage},
    title style={font=\small}
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/citeseer/sage_400.csv} \closedcycle;
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/citeseer/mmlp_sage_400.csv} \closedcycle;

==> communication_costs/citeseer/plot_sage_es.tex <==
\nextgroupplot[
    title = {with early stopping},
    title style={font=\small}
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/citeseer/sage_es.csv} \closedcycle;
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/citeseer/mmlp_sage_es.csv} \closedcycle;

==> communication_costs/cora/plot_cora.tex <==
\begin{figure}[t]
    \begin{tikzpicture}
        \begin{groupplot}[group style = {group size = 6 by 1, horizontal sep = 25pt, vertical sep = 35pt, xlabels at=edge bottom, ylabels at=edge bottom},
                width=1/4.5*\textwidth,
                height = 3.8cm,
                xlabel={Client},
                x label style={font=\small},
                y label style={font=\small}]
            \input{communication_costs/cora/plot_gcn_400.tex}
            \input{communication_costs/cora/plot_gcn_es.tex}
            \input{communication_costs/cora/plot_sage_400.tex}
            \input{communication_costs/cora/plot_sage_es.tex}
            \input{communication_costs/cora/plot_gat_400.tex}
            \input{communication_costs/cora/plot_gat_es.tex}
        \end{groupplot}
        \node at ($(group c2r1) + (2.05cm,-2.4cm)$) {\ref{grouplegend1}};
    \end{tikzpicture}
    \caption{Comparison of data volume transferred for \cora.}
    \label{fig:comm_cora}
\end{figure}

==> communication_costs/cora/plot_gat_400.tex <==
\nextgroupplot[title = {\gat vs \toolgat},
    title style={font=\small},
    ylabel={Data transferred in MB},
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/cora/cora_gat_400.csv} \closedcycle;
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/cora/cora_mmlp_gat_400.csv} \closedcycle;

==> communication_costs/cora/plot_gat_es.tex <==
\nextgroupplot[title = {with early stopping },
    title style={font=\small},
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/cora/cora_gat_es.csv} \closedcycle;
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/cora/cora_mmlp_gat_es.csv} \closedcycle;

==> communication_costs/cora/plot_gat_with_server.tex <==
\nextgroupplot[
    title = {client to server},
    title style={font=\tiny}
]

    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.2, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/cora/cora_mmlp_gat_with_server_400.csv} \closedcycle;
    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/cora/cora_gat_with_server_400.csv} \closedcycle;

==> communication_costs/cora/plot_gcn_400.tex <==

\nextgroupplot[title = {\gcn vs \toolgcn},
    title style={font=\small},
    x tick style={font=\Huge},
    legend style={column sep = 1pt, legend columns = 2, legend to name = grouplegend1, font=\small},
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/cora/cora_gcn_400.csv} \closedcycle;
    \addlegendentry{GNN}
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/cora/cora_mmlp_gcn_400.csv} \closedcycle;
    \addlegendentry{\toolgnn}
    

==> communication_costs/cora/plot_gcn_es.tex <==
\nextgroupplot[title = {with early stopping },
    title style={font=\small},
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/cora/cora_gcn_es.csv} \closedcycle;
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/cora/cora_mmlp_gcn_es.csv} \closedcycle;

==> communication_costs/cora/plot_gcn_with_server_400.tex <==
\nextgroupplot[
    title = {client to server},
    title style={font=\tiny}
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/cora/cora_gcn_with_server_400.csv} \closedcycle;
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/cora/cora_mmlp_gcn_with_server_400.csv} \closedcycle;

==> communication_costs/cora/plot_sage_400.tex <==
\nextgroupplot[
    title = {\sage vs \toolsage},
    title style={font=\small}
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/cora/cora_sage_400.csv} \closedcycle;
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/cora/cora_mmlp_sage_400.csv} \closedcycle;

==> communication_costs/cora/plot_sage_es.tex <==
\nextgroupplot[
    title = {with early stopping},
    title style={font=\small}
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/cora/cora_sage_es.csv} \closedcycle;
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/cora/cora_mmlp_sage_es.csv} \closedcycle;

==> communication_costs/cora/plot_sage_with_server_400.tex <==
\nextgroupplot[
    title = {client to server},
    title style={font=\tiny}
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/cora/cora_sage_with_server_400.csv} \closedcycle;
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/cora/cora_mmlp_sage_with_server_400.csv} \closedcycle;

==> communication_costs/facebook_page/plot_fb.tex <==
\begin{figure}[t]
    \begin{tikzpicture}
        \begin{groupplot}[group style = {group size = 2 by 3, horizontal sep = 25pt, vertical sep = 35pt, xlabels at=edge bottom, ylabels at=edge bottom},
                width=1/3.5*\textwidth,
                height = 3.8cm,
                xlabel={Client},
                x label style={font=\small},
                y label style={font=\small}]
            \input{communication_costs/facebook_page/plot_gcn_400.tex}
            \input{communication_costs/facebook_page/plot_gcn_es.tex}
            \input{communication_costs/facebook_page/plot_sage_400.tex}
            \input{communication_costs/facebook_page/plot_sage_es.tex}
            \input{communication_costs/facebook_page/plot_gat_400.tex}
            \input{communication_costs/facebook_page/plot_gat_es.tex}
        \end{groupplot}
        \node at ($(group c1r3) + (2.05cm,-2.4cm)$) {\ref{grouplegend1}};
    \end{tikzpicture}
    \caption{Comparison of data volume transferred for \fbpage, $400$ rounds on the left and with early stopping on the right.}
    \label{fig:comm_fb}
\end{figure}



==> communication_costs/facebook_page/plot_gat_400.tex <==
\nextgroupplot[title = {\gat vs \toolgat},
    title style={font=\small},
    ylabel = {Data transferred in MB}
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/facebook_page/gat_400.csv} \closedcycle;
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/facebook_page/mmlp_gat_400.csv} \closedcycle;

==> communication_costs/facebook_page/plot_gat_es.tex <==
\nextgroupplot[title = {with early stopping },
    title style={font=\small},
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/facebook_page/gat_es.csv} \closedcycle;
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/facebook_page/mmlp_gat_es.csv} \closedcycle;

==> communication_costs/facebook_page/plot_gcn_400.tex <==

\nextgroupplot[title = {\gcn vs \toolgcn},
    title style={font=\small},
    x tick style={font=\Huge},
    legend style={column sep = 1pt, legend columns = 2, legend to name = grouplegend1, font=\small},
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/facebook_page/gcn_400.csv} \closedcycle;
    \addlegendentry{GNN}
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/facebook_page/mmlp_gcn_400.csv} \closedcycle;
    \addlegendentry{\toolgnn}

==> communication_costs/facebook_page/plot_gcn_es.tex <==
\nextgroupplot[title = {with early stopping },
    title style={font=\small},
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/facebook_page/gcn_es.csv} \closedcycle;
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/facebook_page/mmlp_gcn_es.csv} \closedcycle;

==> communication_costs/facebook_page/plot_sage_400.tex <==
\nextgroupplot[
    title = {\sage vs \toolsage},
    title style={font=\small}
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/facebook_page/sage_400.csv} \closedcycle;
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/facebook_page/mmlp_sage_400.csv} \closedcycle;

==> communication_costs/facebook_page/plot_sage_es.tex <==
\nextgroupplot[
    title = {with early stopping},
    title style={font=\small}
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/facebook_page/sage_es.csv} \closedcycle;
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/facebook_page/mmlp_sage_es.csv} \closedcycle;

==> communication_costs/lastfm/plot_gat_400.tex <==
\nextgroupplot[title = {\gat vs \toolgat},
    title style={font=\small},
    ylabel = {Data transferred in MB}
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/lastfm/gat_400.csv} \closedcycle;
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/lastfm/mmlp_gat_400.csv} \closedcycle;

==> communication_costs/lastfm/plot_gat_es.tex <==
\nextgroupplot[title = {with early stopping },
    title style={font=\small},
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/lastfm/gat_es.csv} \closedcycle;
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/lastfm/mmlp_gat_es.csv} \closedcycle;

==> communication_costs/lastfm/plot_gcn_400.tex <==

\nextgroupplot[title = {\gcn vs \toolgcn},
    title style={font=\small},
    x tick style={font=\Huge},
    legend style={column sep = 1pt, legend columns = 2, legend to name = grouplegend1, font=\small},
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/lastfm/gcn_400.csv} \closedcycle;
    \addlegendentry{GNN}
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/lastfm/mmlp_gcn_400.csv} \closedcycle;
    \addlegendentry{\toolgnn}

==> communication_costs/lastfm/plot_gcn_es.tex <==
\nextgroupplot[title = {with early stopping },
    title style={font=\small},
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/lastfm/gcn_es.csv} \closedcycle;
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/lastfm/mmlp_gcn_es.csv} \closedcycle;

==> communication_costs/lastfm/plot_lastfm.tex <==
\begin{figure}[t]
    \begin{tikzpicture}
        \begin{groupplot}[group style = {group size = 2 by 3, horizontal sep = 25pt, vertical sep = 35pt, xlabels at=edge bottom, ylabels at=edge bottom},
                width=1/3.5*\textwidth,
                height = 3.8cm,
                xlabel={Client},
                x label style={font=\small},
                y label style={font=\small}]
            \input{communication_costs/lastfm/plot_gcn_400.tex}
            \input{communication_costs/lastfm/plot_gcn_es.tex}
            \input{communication_costs/lastfm/plot_sage_400.tex}
            \input{communication_costs/lastfm/plot_sage_es.tex}
            \input{communication_costs/lastfm/plot_gat_400.tex}
            \input{communication_costs/lastfm/plot_gat_es.tex}
        \end{groupplot}
        \node at ($(group c1r3) + (2.05cm,-2.4cm)$) {\ref{grouplegend1}};
    \end{tikzpicture}
    \caption{Comparison of data volume transferred for \lastfm, $400$ rounds on the left and with early stopping on the right.}
    \label{fig:comm_lastfm}
\end{figure}



==> communication_costs/lastfm/plot_sage_400.tex <==
\nextgroupplot[
    title = {\sage vs \toolsage},
    title style={font=\small}
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/lastfm/sage_400.csv} \closedcycle;
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/lastfm/mmlp_sage_400.csv} \closedcycle;

==> communication_costs/lastfm/plot_sage_es.tex <==
\nextgroupplot[
    title = {with early stopping},
    title style={font=\small}
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/lastfm/sage_es.csv} \closedcycle;
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/lastfm/mmlp_sage_es.csv} \closedcycle;

==> communication_costs/pubmed/plot_gat_400.tex <==
\nextgroupplot[title = {\gat vs \toolgat},
    title style={font=\small},
    ylabel = {Data transferred in MB}
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/pubmed/gat_400.csv} \closedcycle;
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/pubmed/mmlp_gat_400.csv} \closedcycle;

==> communication_costs/pubmed/plot_gat_es.tex <==
\nextgroupplot[title = {with early stopping },
    title style={font=\small},
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/pubmed/gat_es.csv} \closedcycle;
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/pubmed/mmlp_gat_es.csv} \closedcycle;

==> communication_costs/pubmed/plot_gcn_400.tex <==

\nextgroupplot[title = {\gcn vs \toolgcn},
    title style={font=\small},
    x tick style={font=\Huge},
    legend style={column sep = 1pt, legend columns = 2, legend to name = grouplegend1, font=\small},
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/pubmed/gcn_400.csv} \closedcycle;
    \addlegendentry{GNN}
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/pubmed/mmlp_gcn_400.csv} \closedcycle;
    \addlegendentry{\toolgnn}

==> communication_costs/pubmed/plot_gcn_es.tex <==
\nextgroupplot[title = {with early stopping },
    title style={font=\small},
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/pubmed/gcn_es.csv} \closedcycle;
    
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/pubmed/mmlp_gcn_es.csv} \closedcycle;

==> communication_costs/pubmed/plot_pubmed.tex <==
\begin{figure}[t]
    \begin{tikzpicture}
        \begin{groupplot}[group style = {group size = 2 by 3, horizontal sep = 25pt, vertical sep = 35pt, xlabels at=edge bottom, ylabels at=edge bottom},
                width=1/3.5*\textwidth,
                height = 3.8cm,
                xlabel={Client},
                x label style={font=\small},
                y label style={font=\small}]
            \input{communication_costs/pubmed/plot_gcn_400.tex}
            \input{communication_costs/pubmed/plot_gcn_es.tex}
            \input{communication_costs/pubmed/plot_sage_400.tex}
            \input{communication_costs/pubmed/plot_sage_es.tex}
            \input{communication_costs/pubmed/plot_gat_400.tex}
            \input{communication_costs/pubmed/plot_gat_es.tex}
        \end{groupplot}
        \node at ($(group c1r3) + (2.05cm,-2.4cm)$) {\ref{grouplegend1}};
    \end{tikzpicture}
    \caption{Comparison of data volume transferred for \pubmed, $400$ rounds on the left and with early stopping on the right.}
    \label{fig:comm_pubmed}
\end{figure}



==> communication_costs/pubmed/plot_sage_400.tex <==
\nextgroupplot[
    title = {\sage vs \toolsage},
    title style={font=\small}
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/pubmed/sage_400.csv} \closedcycle;
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/pubmed/mmlp_sage_400.csv} \closedcycle;

==> communication_costs/pubmed/plot_sage_es.tex <==
\nextgroupplot[
    title = {with early stopping},
    title style={font=\small}
]

    \addplot[smooth, \gnncolor!75!black, fill=\gnncolor, opacity=0.5, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/pubmed/sage_es.csv} \closedcycle;
    \addplot[smooth, \mmlpcolor!75!black, fill=\mmlpcolor, opacity=0.8, mark=., draw] table [x=Sno, y=node, col sep=comma] {communication_costs/pubmed/mmlp_sage_es.csv} \closedcycle;

==> figures/cora_acc_vs_comm_400.tex <==
\nextgroupplot[title = {\cora},
    title style={font=\small},
    xlabel=Communication (MB),
    ylabel=Accuracy,
    error bars/y dir=both, 
    error bars/y explicit,
    xmode=log,
    legend style={column sep = 1pt, legend columns = 6, legend to name = grouplegend1,}
    ]

    \addplot[scatter, only marks, scatter src=explicit symbolic, scatter/classes={
        gcn={mark=square*,blue},
        toolgcn={mark=triangle*,blue},
        sage={mark=square*,red},
        toolsage={mark=triangle*,red},
        gat={mark=square*,black},
        toolgat={mark=triangle*,black}
        }] table[x=communication,y=acc_mean, y error=acc_std,col sep=comma, meta=architecture]{figures/cora_acc_comm.csv};
    \legend{\gcn,\toolgcn,\sage,\toolsage,\gat,\toolgat}

==> figures/facebook_acc_vs_comm_400.tex <==
\nextgroupplot[title = {\fbpage},
    title style={font=\small},
    error bars/y dir=both, 
    error bars/y explicit,
    xmode=log,
    ]

    \addplot[scatter, only marks, scatter src=explicit symbolic, scatter/classes={
        gcn={mark=square*,blue},
        toolgcn={mark=triangle*,blue},
        sage={mark=square*,red},
        toolsage={mark=triangle*,red},
        gat={mark=square*,black},
        toolgat={mark=triangle*,black}
        }] table[x=communication,y=acc_mean, y error=acc_std,col sep=comma, meta=architecture]{figures/facebook_acc_comm.csv};


==> figures/lastfm_acc_vs_comm_400.tex <==
\nextgroupplot[title = {\lastfm},
    title style={font=\small},
    error bars/y dir=both, 
    error bars/y explicit,
    xmode=log,
    ]

    \addplot[scatter, only marks, scatter src=explicit symbolic, scatter/classes={
        gcn={mark=square*,blue},
        toolgcn={mark=triangle*,blue},
        sage={mark=square*,red},
        toolsage={mark=triangle*,red},
        gat={mark=square*,black},
        toolgat={mark=triangle*,black}
        }] table[x=communication,y=acc_mean, y error=acc_std,col sep=comma, meta=architecture]{figures/lastfm_acc_comm.csv};


==> figures/ogbn-products_acc_vs_dv_2.tex <==
\nextgroupplot[title = {Products},
    title style={font=\small},
    xlabel=Communication (Bytes),
    ylabel=Accuracy,
    error bars/y dir=both, 
    error bars/y explicit,
    xmode=log,
    % legend style={column sep = 1pt, legend columns = 6, legend to name = grouplegend1,}
    ]

    \addplot[scatter, only marks, scatter src=explicit symbolic, scatter/classes={
        gcn={mark=triangle*,blue},
        graphsage={mark=triangle*,red},
        gat={mark=triangle*,black},
        baseline1gcn={mark=square*,blue},
        baseline1graphsage={mark=square*,red},
        baseline1gat={mark=square*,black},
        baseline01gcn={mark=star,blue},
        baseline01graphsage={mark=star,red},
        baseline01gat={mark=star,black}
        % baseline001gcn={mark=diamond*,blue},
        % baseline001graphsage={mark=diamond*,red},
        % baseline001gat={mark=diamond*,black}
        }] table[x=communication,y=acc_mean, y error=acc_std,col sep=comma, meta=architecture]{figures/products_dv_2.csv};
    % \legend{\toolgcn,\toolsage,\toolgat,\gcn,\sage,\gat,\gcna, \sagea, \gata 
    % \gcnb, \sageb, \gatb
    % }

==> figures/products_finer_comm_graphsage_2.tex <==
\nextgroupplot[title = {Products},
        title style={font=\small},
        table/col sep=comma,
        ybar stacked,
        ymode=log,
        xtick=data,
        legend style={
            cells={anchor=west},
            legend pos=north west,
        },
        % reverse legend=true,
        % xticklabels from table={figures/ogbn-products-graphsage-2-finer_dv.csv}{architecture},
        xticklabels={\toolsage, \sage, \sagea},
        xticklabel style={text width=2cm,align=center},
        ylabel={Data Volume (in bytes)},
    ]
        \addplot [pattern=crosshatch dots, pattern color=red!60]
            table [col sep=comma, y=message-passing, meta=architecture, x expr=\coordindex]
                {figures/ogbn-products-graphsage-2-finer_dv.csv};
                    \addlegendentry{message passing}
        \addplot [fill=mygray]
            table [col sep=comma, y=total, meta=architecture, x expr=\coordindex]
                {figures/ogbn-products-graphsage-2-finer_dv.csv};
                    \addlegendentry{total}
        


==> figures/products_training_time.tex <==
\nextgroupplot[title = {Products},
        title style={font=\small},
        table/col sep=comma,
        ybar stacked,
        ymode =log,
        xtick=data,
        legend style={
            cells={anchor=west},
            legend pos=north west,
            font=\tiny,
        },
        % reverse legend=true,
        % xticklabels from table={figures/ogbn-products-graphsage-2-finer_dv.csv}{architecture},
        xticklabels={\toolsage, \sage, BNS-SAGE},
        xticklabel style={text width=2cm,align=center, font=\small},
    ]
        \addplot [pattern=crosshatch dots, pattern color=red!60]
            table [col sep=comma, y=message-passing, meta=architecture, x expr=\coordindex]
                {figures/ogbn-products-graphsage-time.csv};
                    \addlegendentry{message-passing}
        \addplot [fill=mygray]
            table [col sep=comma, y=total, meta=architecture, x expr=\coordindex]
                {figures/ogbn-products-graphsage-time.csv};
                    \addlegendentry{total}
        

==> figures/pubmed_acc_vs_comm_400.tex <==
\nextgroupplot[title = {\pubmed},
    title style={font=\small},
    error bars/y dir=both, 
    error bars/y explicit,
    xmode=log,
    ]

    \addplot[scatter, only marks, scatter src=explicit symbolic, scatter/classes={
        gcn={mark=square*,blue},
        toolgcn={mark=triangle*,blue},
        sage={mark=square*,red},
        toolsage={mark=triangle*,red},
        gat={mark=square*,black},
        toolgat={mark=triangle*,black}
        }] table[x=communication,y=acc_mean, y error=acc_std,col sep=comma, meta=architecture]{figures/pubmed_acc_comm.csv};


==> figures/reddit_acc_vs_dv_2.tex <==
\nextgroupplot[title = {Reddit},
    title style={font=\small},
    % xlabel=Communication (Bytes),
    ylabel=Accuracy,
    error bars/y dir=both, 
    error bars/y explicit,
    xmode=log,
    legend style={cells={align=left}, column sep = 0.5pt, legend columns=3, legend to name = grouplegend1,}
    ]

    \addplot[scatter, only marks, scatter src=explicit symbolic, scatter/classes={
        gcn={mark=triangle*,blue},
        graphsage={mark=triangle*,red},
        gat={mark=triangle*,black},
        baseline1gcn={mark=square*,blue},
        baseline1graphsage={mark=square*,red},
        baseline1gat={mark=square*,black},
        baseline01gcn={mark=star,blue},
        baseline01graphsage={mark=star,red},
        baseline01gat={mark=star,black}
        % baseline001gcn={mark=diamond*,blue},
        % baseline001graphsage={mark=diamond*,red},
        % baseline001gat={mark=diamond*,black}
        }] table[x=communication,y=acc_mean, y error=acc_std,col sep=comma, meta=architecture]{figures/reddit_dv_2.csv};
        \addlegendentry{\toolgcn};
        \addlegendentry{\toolsage};
        \addlegendentry{\toolgat};
        \addlegendentry{\gcn};
        \addlegendentry{\sage};
        \addlegendentry{\gat};
        \addlegendentry{\gcna};
        \addlegendentry{\sagea};
        \addlegendentry{\gata};
        
    % \legend{\toolgcn,\toolsage,\toolgat,\\,\gcn,\sage,\gat,\gcna, \sagea, \gata 
    % % \gcnb, \sageb, \gatb
    % }

==> figures/reddit_finer_comm_graphsage_2.tex <==
\nextgroupplot[title = {Reddit},
        title style={font=\small},
        table/col sep=comma,
        ylabel={Data Volume (in bytes)},
        ybar stacked,
        ymode=log,
        xtick=data,
        legend style={
            cells={anchor=west},
            legend pos=north west,
        },
        % reverse legend=true,
        % xticklabels from table={figures/reddit-graphsage-2-finer_dv.csv}{architecture},
        xticklabels={\toolsage, \sage, \sagea},
        xticklabel style={text width=2cm,align=center},
    ]   
        \addplot [pattern=crosshatch dots, pattern color=red!60]
            table [col sep=comma, y=message-passing, meta=architecture, x expr=\coordindex]
                {figures/reddit-graphsage-2-finer_dv.csv};
                    \addlegendentry{message passing}
        \addplot [fill=mygray]
            table [col sep=comma, y=total, meta=architecture, x expr=\coordindex]
                {figures/reddit-graphsage-2-finer_dv.csv};
                    \addlegendentry{total}


==> figures/seer_acc_vs_comm_400.tex <==
\nextgroupplot[title = {\seer},
    title style={font=\small},
    error bars/y dir=both, 
    error bars/y explicit,
    xmode=log,
    ]

    \addplot[scatter, only marks, scatter src=explicit symbolic, scatter/classes={
        gcn={mark=square*,blue},
        toolgcn={mark=triangle*,blue},
        sage={mark=square*,red},
        toolsage={mark=triangle*,red},
        gat={mark=square*,black},
        toolgat={mark=triangle*,black}
        }] table[x=communication,y=acc_mean, y error=acc_std,col sep=comma, meta=architecture]{figures/seer_acc_comm.csv};


==> tables/datastats.tex <==
\begin{table}[ht]
     \centering
    \caption{All datasets' statistics.}
    % \resizebox{\textwidth}{!}{%
    \begin{tabular}{l l l l l l}
        % \multicolumn{6}{c}{Transductive Setting}
        \toprule
        Dataset & Nodes & Edges &  Density & Features & Classes\\ \hline
        \cora   & 2,708 & 10,566 & 0.0015 & 1,433 & 7 \\
        \seer   & 3,327 & 9,104 & 0.0008 & 3,703 & 6 \\
        \pubmed & 19,717 & 88,648 & 0.0002 & 500 & 3 \\
        \fbpage & 22,470 & 	342,004 & 0.0007 & 128 & 4 \\
        \lastfm & 7,624  &  55,612       & 0.0009        &  128    & 16 \\
        \wikicooc & 10,000 & 2,243,042 & 0.0448 & 100 & 5\\
        \romane & 22,662 & 32,927 & 0.0001 & 300 & 18\\ \hline
    \end{tabular}
    % }
    \label{tab:datastats}
\end{table}
